Target-Quality Image Compression with Recurrent, Convolutional Neural Networks

We introduce a stop-code tolerant (SCT) approach to training recurrent convolutional neural networks for lossy image compression. Our methods introduce a multi-pass training method to combine the training goals of high-quality reconstructions in areas around stop-code masking as well as in highly-detailed areas. These methods lead to lower true bitrates for a given recursion count, both pre- and post-entropy coding, even using unstructured LZ77 code compression. The pre-LZ77 gains are achieved by trimming stop codes. The post-LZ77 gains are due to the highly unequal distributions of 0/1 codes from the SCT architectures. With these code compressions, the SCT architecture maintains or exceeds the image quality at all compression rates compared to JPEG and to RNN auto-encoders across the Kodak dataset. In addition, the SCT coding results in lower variance in image quality across the extent of the image, a characteristic that has been shown to be important in human ratings of image quality

==> orphaned.tex <==
Our approach uses multiple
techniques.  We introduce new terms to our training loss to encourage
the encoder network to output zeros in the masked areas and we replace
the codes that are produced in these masked areas with zeros before
providing them to the decoder network.  We also run each training
example through each iteration of the network twice, one time
with the correct masking (as dictated by our target quality), so that
the network will be rewarded for providing sharp reconstructions under
normal conditions, and one time with the best
current-reconstruction areas forced into the `masked' condition, so
that the network will be rewarded for finding ways to avoid blocking
artifacts.


-------------------


In the non-EST approach, the input image is passed through a feed-forward
convolutional layer, with spatial downsampling on the output, followed
by several layers of LSTMs, each with downsampling on the output.  In
this way, each $16 \times 16$ spatial `tile' in the input image (and,
after the
decoder, in the reconstructed image) corresponds to a stack of outputs
from the encoder network, where the height of the stack is determined
by the
output depth of the final layer of the encoder.  The encoder output is
then passed into a binarizer which does depth-only mixing down to a
depth equal to the number of bits that the system will output for that
tile, followed by mapping to -1 or 1.  It is the number of bi-level
values output from the binarizer that defines the nominal bit-rate.
The binary codes are input into a 'decoder' network, consisting of a
single feed-forward layer followed by several LSTM layers.  After each
of these layers, the
decoder uses 'depth-to-space' shuffling to increase the spatial
resolution of the reconstruction.  There is one final layer of
depth-only mixing to create the output reconstruction from the
decoder.




-------------------


[ After: Another research direction is to take this same early-stopping idea
and apply it to non-recurrent auto-encoders.  This would require
assigning ``priority'' to different sections of the auto-encoder's
bottleneck.]

  This research would need to decide how best to
communicate stopping: whether to send the information with the number
of used bits or, if not, how many bits to group together to create a
stop code and whether that is a ``fixed-frame'' stop code (e.g., it
must be all zeros for bits $32*k$ through $32*k+31$ or a
``sliding-frame'' stop code (e.g., any sequence of 32 zero bits
indicates a stop).

